Alignment of Magnetized Accretion Disks and Relativistic Jets with Spinning Black Holes

Accreting black holes (BHs) produce intense radiation and powerful relativistic jets, which are affected by the BH's spin magnitude and direction. While thin disks might align with the BH spin axis via the Bardeen-Petterson effect, this does not apply to jet systems with thick disks. We used fully three-dimensional general relativistic magnetohydrodynamical simulations to study accreting BHs with various BH spin vectors and disk thicknesses with magnetic flux reaching saturation. Our simulations reveal a "magneto-spin alignment" mechanism that causes magnetized disks and jets to align with the BH spin near BHs and further away to reorient with the outer disk. This mechanism has implications for the evolution of BH mass and spin, BH feedback on host galaxies, and resolved BH images for SgrA* and M87.

==> authorssup.tex <==

\author
{Jonathan C. McKinney$^{\ast}$, Alexander Tchekhovskoy, Roger D. Blandford\\
\normalsize{$^{\ast}$To whom correspondence should be addressed; E-mail:  jcm@umd.edu .}
}



==> suptitle.tex <==
\title{{\Large Supplementary Materials for}\\[0.3in]\mytitle}

